Decisions and Performance Under Bounded Rationality: A Computational Benchmarking Approach

This paper presents a novel approach to analyze human decision-making that involves comparing the behavior of professional chess players relative to a computational benchmark of cognitively bounded rationality. This benchmark is constructed using algorithms of modern chess engines and allows investigating behavior at the level of individual move-by-move observations, thus representing a natural benchmark for computationally bounded optimization. The analysis delivers novel insights by isolating deviations from this benchmark of bounded rationality as well as their causes and consequences for performance. The findings document the existence of several distinct dimensions of behavioral deviations, which are related to asymmetric positional evaluation in terms of losses and gains, time pressure, fatigue, and complexity. The results also document that deviations from the benchmark do not necessarily entail worse performance. Faster decisions are associated with more frequent deviations from the benchmark, yet they are also associated with better performance. The findings are consistent with an important influence of intuition and experience, thereby shedding new light on the recent debate about computational rationality in cognitive processes.

==> Summary_Tournaments_unedited.tex <==
tournament\_name&No.&\% \\
\hline
Armenian Championship&60.0&3.0 \\
Danzhou&42.0&2.1 \\
FIDE Grand Prix&281.0&14.2 \\
French Championship&62.0&3.1 \\
Lake Sevan&68.0&3.4 \\
Norway Chess&84.0&4.2 \\
Other Invited Tournament&307.0&15.5 \\
Other National Championship&114.0&5.8 \\
Poikovsky&80.0&4.0 \\
Russian Championship&165.0&8.3 \\
Shamkir&76.0&3.8 \\
U.S. Championship&114.0&5.8 \\
Ukrainian Championship&77.0&3.9 \\
Wijk aan Zee&452.0&22.8 \\
Total&1,982.0&100.0 \\

